Ballistic Josephson junctions in edge-contacted graphene

Hybrid graphene-superconductor devices have attracted much attention since the early days of graphene research. So far, these studies have been limited to the case of diffusive transport through graphene with poorly defined and modest quality graphene-superconductor interfaces, usually combined with small critical magnetic fields of the superconducting electrodes. Here we report graphene based Josephson junctions with one-dimensional edge contacts of Molybdenum Rhenium. The contacts exhibit a well defined, transparent interface to the graphene, have a critical magnetic field of 8 Tesla at 4 Kelvin and the graphene has a high quality due to its encapsulation in hexagonal boron nitride. This allows us to study and exploit graphene Josephson junctions in a new regime, characterized by ballistic transport. We find that the critical current oscillates with the carrier density due to phase coherent interference of the electrons and holes that carry the supercurrent caused by the formation of a Fabry-P\'{e}rot cavity. Furthermore, relatively large supercurrents are observed over unprecedented long distances of up to 1.5 $\mu$m. Finally, in the quantum Hall regime we observe broken symmetry states while the contacts remain superconducting. These achievements open up new avenues to exploit the Dirac nature of graphene in interaction with the superconducting state.

==> definitions.tex <==
\usepackage[version=3]{mhchem} % Formula subscripts using \ce{}
%\usepackage{color}
\usepackage{xr}
\usepackage[english]{babel}
\usepackage{natbib}
\usepackage{microtype}
%\bibliographystyle{apsrev4-1}
\bibliographystyle{unsrt}
\usepackage{hyperref}
\usepackage{MnSymbol}%
\usepackage{wasysym}%
\hypersetup{colorlinks=true,citecolor=blue}
\graphicspath{{./images/}}

\newcommand{\thesis}{letter}
\newcommand*{\mycommand}[1]{\texttt{\emph{#1}}}
\newcommand{\unit}{\ \mathrm}
\newcommand{\temp}[1]{$#1~^{\circ}$C}
\newcommand{\degree}{\ensuremath{^{\circ}}}
%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
%\newcommand{\green}[1]{\textcolor{green}{#1}}

\newcommand{\GrapheneJJliterature}{Heersche2007, Du2008, Miao2009, Girit2009, OAristizabal2009, Kanda2010, Choi2010, Borzenets2011, Coskun2011, Lee2011, Rickhaus2012, Popinciuc2012,Komatsu2012, Mizuno2013, Voutilainen2011, JeongChoi2011, Borzenetz2013, Choi2013}

\newcommand{\Delft}{Kavli Institute of Nanoscience, Delft University of Technology, 2600 GA Delft, The Netherlands}
\newcommand{\Leiden}{Instituut-Lorentz, Universiteit Leiden, P.O. Box 9506, 2300 RA
Leiden, The Netherlands}
\newcommand{\NIMS}{Advanced Materials Laboratory, National Institute for Materials Science, 1-1 Namiki, Tsukuba, 305-0044, Japan}
\newcommand{\Moscow}{Laboratory for Quantum Limited Devices, Physics Department,
Moscow State Pedagogical University, 29 Malaya Pirogovskaya St., Moscow, 119992, Russia}
\newcommand{\Wurzburg}{Institute for Theoretical Physics and Astrophysics,
University W\"{u}rzburg, Am Hubland, 97074 W\"{u}rzburg, Germany}

%\newcommand{\TITLE}{Long-distance ballistic Josephson supercurrent in high quality edge-contacted graphene}
%\newcommand{\TITLE}{Micron scale ballistic Josephson junctions in high quality edge-contacted graphene}
%\newcommand{\TITLE}{Superconducting edge-contacts to graphene}
\newcommand{\TITLE}{Ballistic Josephson junctions in edge-contacted graphene}

